Large-scale Cloze Test Dataset Created by Teachers

Cloze tests are widely adopted in language exams to evaluate students' language proficiency. In this paper, we propose the first large-scale human-created cloze test dataset CLOTH, containing questions used in middle-school and high-school language exams. With missing blanks carefully created by teachers and candidate choices purposely designed to be nuanced, CLOTH requires a deeper language understanding and a wider attention span than previously automatically-generated cloze datasets. We test the performance of dedicatedly designed baseline models including a language model trained on the One Billion Word Corpus and show humans outperform them by a significant margin. We investigate the source of the performance gap, trace model deficiencies to some distinct properties of CLOTH, and identify the limited ability of comprehending the long-term context to be the key bottleneck.

==> table/multiple_question.tex <==
\iffalse
\begin{table*}[ht]
\begin{tabular}{l|cccc}
\hline
Dataset & Multi-answer & \# choices for multi-answer & Single-answer acc & Multi-answer acc  \\ \hline
\name & 0.302 & 3.41 & 0.765 & 0.589   \\ 
\namem & 0.245 & 3.46 & 0.830 & 0.589 \\
\nameh & 0.325 & 3.39 & 0.740 & 0.589 \\
\hline
\end{tabular}
\caption{Human behavior study when only one sentence is given as context}
\label{tab:multiple_answer}
\end{table*}
\fi

\begin{table*}[ht]
\centering
\begin{tabular}{l|ccc}
\hline
 & \name & \namem & \nameh \\ \hline
Question proportion& 0.302 & 0.245 & 0.325 \\
Average \# of possible answers & 3.41 & 3.46 & 3.39 \\
Best guess accuracy & 0.589 & 0.589 & 0.589  \\
\hline
\end{tabular}
\caption{The statistics of questions with multiple possible answers when only one sentence is given as context}
\label{tab:multiple_answer}
\end{table*}
